Streaming Detection of Queried Event Start

Robotics, autonomous driving, augmented reality, and many embodied computer vision applications must quickly react to user-defined events unfolding in real time. We address this setting by proposing a novel task for multimodal video understanding-Streaming Detection of Queried Event Start (SDQES). The goal of SDQES is to identify the beginning of a complex event as described by a natural language query, with high accuracy and low latency. We introduce a new benchmark based on the Ego4D dataset, as well as new task-specific metrics to study streaming multimodal detection of diverse events in an egocentric video setting. Inspired by parameter-efficient fine-tuning methods in NLP and for video tasks, we propose adapter-based baselines that enable image-to-video transfer learning, allowing for efficient online video modeling. We evaluate three vision-language backbones and three adapter architectures on both short-clip and untrimmed video settings.

==> Figures/sampling_metrics.tex <==
\begin{figure}[t]%[ht]
\centering
\includegraphics[width=0.7\columnwidth,trim={6cm 3.3cm 6.7cm 3cm},clip]{Figures/fig4_samplingmetrics_v0.pdf}
% \vskip -0.1in
\caption{ \textbf{\task Streaming Recall Metric.} Horizontal axis is time, vertical axis is per-frame detection score, red line is detection threshold, yellow window is temporal threshold from the ground-truth within which a detection is considered correct.
The Streaming Recall (SR) metric measures streaming accuracy with observation latency constraints, considering only the first $k$ predicted query starts. \textit{(top)} For low $k$, models with high false positive rates perform badly. \textit{(middle)} Second, window width controls maximum accepted latency. \textit{(bottom)} As more predictions are considered and windows are widened the metric value increases. For details on SR and supporting metrics (\eg SMD), see Sec.~\ref{sec_technical_approach_metrics}. }
\label{fig_samplingmetrics}
\vskip -0.1in
\end{figure}
